CogVLM: Visual Expert for Pretrained Language Models

We introduce CogVLM, a powerful open-source visual language foundation model. Different from the popular shallow alignment method which maps image features into the input space of language model, CogVLM bridges the gap between the frozen pretrained language model and image encoder by a trainable visual expert module in the attention and FFN layers. As a result, CogVLM enables deep fusion of vision language features without sacrificing any performance on NLP tasks. CogVLM-17B achieves state-of-the-art performance on 10 classic cross-modal benchmarks, including NoCaps, Flicker30k captioning, RefCOCO, RefCOCO+, RefCOCOg, Visual7W, GQA, ScienceQA, VizWiz VQA and TDIUC, and ranks the 2nd on VQAv2, OKVQA, TextVQA, COCO captioning, etc., surpassing or matching PaLI-X 55B. Codes and checkpoints are available at https://github.com/THUDM/CogVLM.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/VQA.tex <==
\begin{table*}[htbp]
  \vspace*{-0.1cm}
 % \caption{Performance comparison of state-of-the-art visual question answering methods on various datasets. * refers to few-shot or zero-shot setting. }
 \caption{Performance on Visual Question Answering benchmarks, where the results labeled with * refers to the few-shot or zero-shot setting. }
  \resizebox{\textwidth}{!}{%
  \centering
  \renewcommand{\arraystretch}{1.15}
  \setlength{\tabcolsep}{1pt}
  \small
  {
    \begin{tabular}{lp{0.8cm}p{0.8cm}cp{1.2cm}p{0.8cm}p{0.8cm}>{\centering}p{1.2cm}>{\centering}p{1.2cm}c}
    \toprule
    \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{p{0.4cm}}{\textbf{VQAv2}} & \multicolumn{1}{r}{\textbf{OKVQA}} & \multicolumn{1}{c}{\textbf{GQA}} & \multicolumn{2}{l}{\textbf{VizWizQA}} & \multicolumn{1}{c}{\textbf{OCRVQA}} & \multicolumn{1}{c}{\textbf{TextVQA}} & \textbf{SciQA}\\
    \cmidrule(r{10pt}){2-3} \cmidrule(r){4-4} \cmidrule(r){5-5} \cmidrule(r){6-7} \cmidrule(r){8-8} \cmidrule(r){9-9} \cmidrule(r){10-10}
    & test-dev & test-std & val & test-balanced & test-dev & test-std & test & test & IMG \\
        \midrule
        \multicolumn{3}{l}{\it{Closed-ended classification models}} \\
        \hline
        SimVLM~\citep{wang2021simvlm} & 80.0 & 80.3 & - & - & - & - & -  & - & -\\
        CoCa~\citep{yu2022coca} & 82.3 & 82.3 & - & - & - & - & -  & - & -\\
        OFA~\citep{wang2022ofa} & 82.0 & 82.0 & - & - & - & - & -  & - & -\\
        BEiT-3~\cite{wang2022image} & 84.2 & 84.0 & - & - & - & -  & - & - & -\\
        \hline
        \multicolumn{3}{l}{\it{Open-ended generation models}} \\
        \hline
        GIT~\citep{wang2022git} &  78.6 & 78.8 & - & - & 68.0 & 67.5 & 68.1  & 59.8 & -\\
        GIT2~\citep{wang2022git} &  81.7 & 81.9 & - & - & 71.0 & 70.1 & 70.3  & 67.3 & -\\
        Flamingo-80B~\citep{alayrac2022flamingo} & 82.0 & 82.1 & 57.8* & - & 65.7 & 65.4 & -  & 54.1 & -\\
        BLIP-2~\citep{li2023blip} & 82.2 & 82.3 & 59.3 & 44.7* & - & - & 72.7  & - & 89.5\\
        InstructBLIP~\citep{dai2023instructblip} & - & - & 62.1 & \underline{49.5}* & 34.5* & - & 73.3  & 50.7* & 90.7\\
        PaLI-17B~\cite{chen2022pali} & 84.3 & 84.3 & 64.5 & - & 71.6 & 70.7 & -  & 58.8 & -\\
        PaLI-X-55B~\citep{chen2023pali} & \textbf{86.0} & \textbf{86.1} & \textbf{66.1} & - & \underline{72.6} & \underline{70.9} & \textbf{75.0}  & \textbf{71.4} & -\\
        PaLM-E-84B~\citep{driess2023palm} & 80.5 & - & 63.3 & - & - & - & - & - & -\\
        % Qwen-VL  & 79.5 & - & 58.6 & \textbf{59.3} & 38.9* & - & \textbf{75.7} & 63.8  \\
        \hline
        CogVLM (ours) & \underline{84.7} & \underline{84.7} & \underline{64.7} & \textbf{65.2} & \textbf{76.4} & \textbf{75.8} & \underline{74.5}  & \underline{69.7} & \textbf{92.7}\\
%     Human & 91.6 & 14.2 & 85.3 & 14.6 & 87.1 & 14.2 & - \\
%     VinVL & 78.0 & 11.5 & 92.5 & 13.1 & 94.3 & 13.1 & - \\
    \bottomrule
    \end{tabular}
  }
 }
    % \vspace{-2mm}
 % \caption{Performance comparison of state-of-the-art visual question answering methods on various datasets. * refers to few-shot or zero-shot setting. }
  \label{vqa}
\end{table*}

% TextVQA: (without OCR pipeline input); TextVQA: (without OCR pipeline input); InstructBlip reported that BLIP-2 after ft: OCRVQA 72.7, OKVQA 59.3; BLIP-2 only report zero-shot on   OKVQA  (45.9); \hwy{generalist zero-shot}

% Flamingto OKVQA 32 shot, others 0 shot


==> tables/chat.tex <==
% \begin{table*}[htbp]
%  \caption{Evaluation results on TouchStone in English.}
%   \resizebox{\textwidth}{!}{%
%   \centering
%   \renewcommand{\arraystretch}{1.15}
%   \setlength{\tabcolsep}{3pt}
%   \small
%   {
%     \begin{tabular}{@{}l|cccccccc@{}}
%     \toprule
%     \textbf{Method} & MiniGPT4 & InstructBLIP & LLaMA-AdapterV2 & LLaVA & mPLUG-Owl & Qwen-VL-Chat & \textbf{CogVLM-Chat} \\
%     \midrule
%     \textbf{Score} & 531.7 & 552.4 & 590.1 & 602.7 & 605.4 & 645.4 & \textbf{651.5}  \\
%     \bottomrule
%     \end{tabular}
%   }
%  }
% \end{table*}

% \begin{table*}[htbp]
%  \caption{Evaluation results on TouchStone in English.}
%   \centering
%   % \renewcommand{\arraystretch}{1.15}
%   % \setlength{\tabcolsep}{3pt}
%   \small
%   {
%     \begin{tabular}{l|c}
%     \toprule
%     Method & {Score}  \\
%     \midrule
%     MiniGPT4 \citep{minigpt4} & 531.7 \\
%     InstructBLIP \citep{dai2023instructblip} & 552.4 \\
%     LLaMA-AdapterV2 \citep{gao2023llamaadapterv2} & 590.1 \\
%     LLaVA \citep{liu2023llava} & 602.7 \\
%     mPLUG-Owl \citep{ye2023mplug} & 605.4 \\
%     Qwen-VL-Chat \citep{bai2023qwen} & 645.4 \\
%     \midrule
%     \textbf{CogVLM-Chat} & \textbf{651.5} \\
%     \bottomrule
%     \end{tabular}
%   }
% \label{tab:chat}
% \end{table*}

    \begin{table}[ht]
  \caption{Evaluation results on TouchStone in English.}
  \renewcommand{\arraystretch}{1.15}
  \resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccccccc}
\toprule
\textbf{Models} & MiniGPT4 & InstructBLIP & LLaMA-AdapterV2 & LLaVA & mPLUG-Owl & Qwen-VL-Chat & \textbf{CogVLM-Chat} \\ \midrule
\textbf{Score}  & 531.7    & 552.4        & 590.1           & 602.7 & 605.4     & 645.4        & \textbf{662.6}     \\ \bottomrule
\end{tabular}
\label{tab:chat}
}
\end{table}


==> tables/tdiuc.tex <==
% \begin{table}
%       % \resizebox{\textwidth}{!}{%
%       \centering
%       \renewcommand{\arraystretch}{1.15}
%       \setlength{\tabcolsep}{3pt}
%       \small
%       {
%         \begin{tabular}{@{}lccccccccc@{}}
%         \toprule
%         \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Subject}} & \multicolumn{3}{c}{\textbf{Context Modality}} & \multicolumn{2}{c}{\textbf{Grade}} & \multicolumn{1}{c}{\textbf{Average}} \\
%         \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-9} \cmidrule(r){10-10} 
%         & NAT & SOC & LAN & TXT & IMG & NO & G1-6 & G7-12 & Average \\
%             \midrule
%             \multicolumn{3}{l}{\it{Zero-shot}} \\
%             \hline
%             BLIP-2 (Vicuna-13B) & - & - & - & - & 61.0 & - & -  & -  & -  \\
%             InstructBLIP (Vicuna-13B) & - & - & - & - & 63.1 & - & -  & -  & - \\
%             Qwen-VL (Qwen01B) & - & - & - & - & 67.1 & - & -  & -  & - \\
%             Qwen-VL-Chat & - & - & - & - & 68.2 & -  & - & -  & - \\
%             \hline
%             \multicolumn{3}{l}{\it{Fine-tuning}} \\
%             \hline
%             LLaVA+GPT-4 (judge) &  91.56 & 96.74 & 91.09 & 90.62 & 88.99 & 93.52 & 92.73  & 92.16 & 92.53\\
%             BLIP-2 (FlanT5$_{XXL}$) &  - & - & - & - & 89.5 & - & -  & - & - \\
%             InstructBLIP (FlanT5$_{XXL}$) &  - & - & - & - & 90.7 & - & -  & - & -\\
%             LLaVAR &  91.79 & 93.81 & 88.73 & 90.57 & 88.70 & 91.57 & 91.30  & 91.63 & 91.42 \\
%             CogVLM (ours) & 90.49 & 97.38 & 72.73 & 91.4 & 92.71 & 90.87 & 93.0  & 92.01 & \textbf{91.74} \\
%         \bottomrule
%         \end{tabular}
%       }
%      % }
%         \vspace{-2mm}
%      \caption{Performance comparison on ScienceQA test set with different partitions.}
%     \end{table}

    
% \begin{minipage}{\textwidth}
  % \begin{minipage}[b]{0.6\textwidth}
  %   % \centering
  %   \captionof{table}{Performance comparison on ScienceQA test set with different partitions.}
  %     \resizebox{0.98\textwidth}{!}{%
  %     \renewcommand{\arraystretch}{1.15}
  %     \setlength{\tabcolsep}{3pt}
  %     \small
  %     {
  %       \begin{tabular}{@{}lccccccc@{}}
  %       \toprule
  %       \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Subject}} & \multicolumn{1}{c}{\textbf{Modality}} & \multicolumn{1}{c}{\textbf{Average}} \\
  %       \cmidrule(r){2-4} \cmidrule(r){5-5} \cmidrule(r){6-6} 
  %       & NAT & SOC & LAN & IMG & Average \\
  %           \midrule
  %           \multicolumn{3}{l}{\it{Zero-shot}} \\
  %           \hline
  %           BLIP-2 (Vicuna-13B) & - &  - & - & 61.0 & -  \\
  %           InstructBLIP (Vicuna-13B) & - & - & - & 63.1 & -\\
  %           Qwen-VL & - &  - & - & 67.1 & -  \\
  %           % Qwen-VL-Chat & - & - &  - & 68.2 & -  \\
  %           \hline
  %           \multicolumn{3}{l}{\it{Fine-tuning}} \\
  %           \hline
  %           LLaVA &  90.36 & 95.95 & 88.00 & 88.00 &  90.92\\
  %           BLIP-2 (FlanT5$_{XXL}$) &  - & - &- & 89.5 & -  \\
  %           InstructBLIP (FlanT5$_{XXL}$) & - & - & - & 90.7 & - \\
  %           LLaVAR &  91.79 & 93.81 & 88.73  & 88.70  & 91.42 \\
  %           CogVLM (ours) & 90.49 & \textbf{97.38} & 72.73 & \textbf{92.71} & \textbf{91.74} \\
  %       \bottomrule
  %       \end{tabular}
  %     }
  %    }
  %    % \caption{Performance comparison on ScienceQA test set with different partitions.}
  %   \label{tab:perform_sciqa}
  %   % \vspace{2pt}
  %   % \captionof{table}{Performance comparison on ScienceQA test set with different partitions.}
  % \end{minipage}\hspace{-8pt}
  % \hfill
  % \begin{minipage}[b]{0.4\textwidth}
    % \centering
    % \includegraphics[scale=0.4]{figures/tdiuc.pdf}
    % \caption{Caption}
    % \label{fig:perform_tdiuc}
    % \vspace{-24pt}
    % \captionof{figure}{Performance on TDIUC.}
    % \vspace{5pt}
  % \end{minipage}
% \end{minipage}


\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figures/tdiuc.pdf}
    \caption{Performance on TDIUC benchmark with fine-grained question classes.}
    \label{fig:perform_tdiuc}
\end{figure}
